DynaSLAM II: Tightly-Coupled Multi-Object Tracking and SLAM

The assumption of scene rigidity is common in visual SLAM algorithms. However, it limits their applicability in populated real-world environments. Furthermore, most scenarios including autonomous driving, multi-robot collaboration and augmented/virtual reality, require explicit motion information of the surroundings to help with decision making and scene understanding. We present in this paper DynaSLAM II, a visual SLAM system for stereo and RGB-D configurations that tightly integrates the multi-object tracking capability. DynaSLAM II makes use of instance semantic segmentation and of ORB features to track dynamic objects. The structure of the static scene and of the dynamic objects is optimized jointly with the trajectories of both the camera and the moving agents within a novel bundle adjustment proposal. The 3D bounding boxes of the objects are also estimated and loosely optimized within a fixed temporal window. We demonstrate that tracking dynamic objects does not only provide rich clues for scene understanding but is also beneficial for camera tracking. The project code will be released upon acceptance.

==> chapters/extra_stuff.tex <==
\begin{equation}
    \theta_{repr} = \{\textbf{T}^{i}_{\mathtt{CW}}, \textbf{X}^{j}_\mathtt{O}, \textbf{T}^{k,i}_{\mathtt{WO}}\}, \quad
    \hat{\theta}_{repr} = \{\hat{\textbf{T}}^{i}_{\mathtt{CW}}, \hat{\textbf{X}}^{j}_\mathtt{O},  \hat{\textbf{T}}^{k,i}_{\mathtt{WO}}\}
\end{equation}

\begin{equation}\label{eqn: rigid_error}
\textbf{e}_{\textbf{vcte,XYZ}}^{i,j,k} = (\textbf{T}_{\mathtt{WO}}^{k,i} - \textbf{T}_{\mathtt{WO}}^{k,i+1} \dot{\textbf{T}}_{\mathtt{OO}_k}^{k,i} \Delta{t}_{i, i+1}) \textbf{X}_{\mathtt{O}}^{j}
\end{equation}

\begin{equation}\label{eqn: solid_rigid}
    \hat{\theta}_{v} =
    \argmin \limits_{\theta_{v}} \sum_{i=1}^n \sum_{j=1}^m \sum_{k=1}^p \rho(\|\textbf{e}_{\textbf{vcte,XYZ}}^{i,j,k}\|^{2}_{\Sigma_{i}^{j}})
\end{equation}

\begin{equation}
    \theta_{v} = \{\textbf{T}_\mathtt{WO}^{k,i}, \textbf{T}_\mathtt{WO}^{k,i+1}, \textbf{X}_{\mathtt{O}}^{j}, \dot{\textbf{T}}_{\mathtt{OO}_k}^{k,i}\},
    \hat{\theta}_{v} =\{\hat{\textbf{T}}_\mathtt{WO}^{k,i}, \hat{\textbf{T}}_\mathtt{WO}^{k,i+1}, \hat{\textbf{X}}_{\mathtt{O}}^{j}, \hat{\dot{\textbf{T}}}_{\mathtt{OO}_k}^{k,i}\}
\end{equation}

\begin{equation}\label{eqn:dT_dt}
    \dot{\textbf{T}}_{\mathtt{OO}_k}^{k,i} = 
    \begin{bmatrix}
     \textbf{I}_{3} + [\textbf{w}^{k,i}_{\mathtt{OO}_k}]_{\times} & | & \textbf{v}^{k,i}_{\mathtt{OO}_k} \\ 
     \cmidrule(lr){1-3}
     \textbf{0}_{1 \times 3} & | & 1
    \end{bmatrix}
\end{equation}

\begin{equation}\label{eqn:w_cte}
    (\hat{\textbf{w}}^{k,i+1}_{\mathtt{OO}_k}, \hat{\textbf{w}}^{k,i}_{\mathtt{OO}_k}) = \argmin \limits_{\textbf{w}^{k,i+1}_{\mathtt{OO}_k}, \textbf{w}^{k,i}_{\mathtt{OO}_k}} 
    \sum_{i=1}^n \sum_{k=1}^p
    \rho(\|\textbf{w}^{k,i+1}_{\mathtt{OO}_k} - \textbf{w}^{k,i}_{\mathtt{OO}_k}\|^{2})
\end{equation}

\begin{equation}\label{eqn:v_cte}
    (\hat{\textbf{v}}^{k,i+1}_{\mathtt{OO}_k}, \hat{\textbf{v}}^{k,i}_{\mathtt{OO}_k}) = \argmin \limits_{\textbf{v}^{k,i+1}_{\mathtt{OO}_k}, \textbf{v}^{k,i}_{\mathtt{OO}_k}} 
    \sum_{i=1}^n \sum_{k=1}^p
    \rho(\|\textbf{v}^{k,i+1}_{\mathtt{OO}_k} - \textbf{v}^{k,i}_{\mathtt{OO}_k}\|^{2})
\end{equation}


\subsection{Exp approximation}
Ecuacion \ref{eqn: rigid_error}, la reescribiria:
\begin{equation}
\textbf{e}_{\textbf{vcte,XYZ}}^{i,j,k} = (\textbf{T}_{\mathtt{WO}}^{k,i+1} - \textbf{T}_{\mathtt{WO}}^{k,i} \Delta \textbf{T}_{\mathtt{O}_k}^{i,i+1} ) \textbf{X}_{\mathtt{O}}^{j}
\end{equation}
Donde $\Delta \textbf{T}_{\mathtt{O}_k}^{i,i+1}$ es la transformacion desde el instante $i+1$ al instante $i$ para el objeto $k$, que se puede reescribir como:
\begin{equation}
\Delta \textbf{T}_{\mathtt{O}_k}^{i,i+1} (\mathbf{w}_i,\mathbf{v}_i) = \left( \begin{array}{cc}
    \text{Exp}(\mathbf{w}_i \Delta t_{i,i+1}) & \mathbf{v}_i \Delta t_{i,i+1}) \\
    \mathbf{0}_{1 \times 3} & 1
\end{array}\right) 
\end{equation}
Suponer que $\mathbf{w}_i \Delta t$ es pequeno y hacer directamente la aproximacion del $\text{Exp}(u)=I+[u]_\times$ para calcular de manera sencilla las derivadas puede que no sea lo correcto. Por ejemplo, si se quiere calcular la derivada de este termino respezto a la velocidad angular, lo mejor seria:
\begin{equation}
\Delta \textbf{T}_{\mathtt{O}_k}^{i,i+1} (\mathbf{w}_i + \delta \mathbf{w}_i ,\mathbf{v}_i) \approx \left( \begin{array}{cc}
    \text{Exp}(\mathbf{w}_i \Delta t)\text{Exp}(\mathbf{J}_r(\mathbf{w}_i \Delta t)\delta \mathbf{w}_i \Delta t) & \mathbf{v}_i \Delta t) \\
    \mathbf{0}_{1 \times 3} & 1
\end{array}\right) 
\end{equation}
Donde he usado la expresion 7 (right jacobian) del arxiv "on manifolds preintegration..." de Foster. Ahora si que se puede suponer que $\mathbf{J}_r(\mathbf{w}_i \Delta t)\delta \mathbf{w}_i \Delta t$ es pequeno, y entonces:
\begin{equation}
\Delta \textbf{T}_{\mathtt{O}_k}^{i,i+1} (\mathbf{w}_i + \delta \mathbf{w}_i ,\mathbf{v}_i) \approx \left( \begin{array}{cc}
    \text{Exp}(\mathbf{w}_i \Delta t)(\mathbf{I} + [\mathbf{J}_r(\mathbf{w}_i \Delta t)\delta \mathbf{w}_i \Delta t]_{\times}) & \mathbf{v}_i \Delta t) \\
    \mathbf{0}_{1 \times 3} & 1
\end{array}\right) 
\end{equation}
Pudiendo calcular la derivada del error respecto a la velocidad angular, $\frac{\partial \textbf{e}_{\textbf{vcte,XYZ}}^{i,j,k}}{\delta \mathbf{w}_i}$ . De todas formas, igual la aproximación inicial no es del todo mala, habria que comparar los valores obtenidos por derivacion numerica (dejar el metodo linearizeoplus sin implementar y que coja el de la clase base g2o::BaseMultiEdge) con los analiticos. 

\subsection{information matrix}
Para la matriz de informacion no se me ocurre como normalizarla. Sin embargo, si que pienso que el error del modelo de velocidad constante (ecuaciones \ref{eqn:w_cte} y \ref{eqn:v_cte}) esta definido por unidad de tiempo. Es decir, si para la velocidad en dos instantes separados una unidad de tiempo se tiene:
\begin{equation}
    \mathbf{v}(t+1)-\mathbf{v}(t) = \eta \sim \mathcal{N}(0,\sigma^2_v)
\end{equation}
Para el caso de dos keyframes separados un tiempo $\Delta_{i,i+1}$:
\begin{equation}
    \mathbf{v}_{i+1}-\mathbf{v}_i = \sum_{i}^{i+1} \eta = \eta_{i,i+1} \sim \mathcal{N}(0,\Delta t_{i,i+1}\sigma^2_v)
\end{equation}
Por lo que habría que escalar la matriz de informacion por $1/\Delta t_{i,i+1}$

In the case in which map points are dynamic, we have modeled their 3D positions as referred to their object coordinates system, instead of to the world one. 
%
The position of the points is fixed with respect to their object, and it is the object's pose which varies along time. 
%
The reprojection error $\mathbf{e}_{\mathbf{repr}}^{i,j,k}$ for a $3D$ point $j$ belonging to an object $k$ observed by the camera $i$ can therefore be formulated as
%
where $\mathbf{T}_\mathtt{WO}^{k,i} \in \text{SE}(3)$ is the inverse pose of the object $k$ in the world coordinates when the camera $i$ is observing it, and $\mathbf{X}_\mathtt{O}^{j,k} \in \mathbb{R}^3$ represents the $3D$ coordinates of the point $j$ in its object reference $k$. 
%
$\mathbf{x}_{i}^{j} \in \mathbb{R}^3$ stands for the observation in the camera $i$ of the point $j$. 
%
Eqn.~\ref{eqn: stereo_projection} represents the reprojection function for a rectified stereo camera with focal length $(f_x, f_y)$, optical center $(c_x, c_y)$ and horizontal baseline $b$. 
%
Given these camera intrinsics, $\pi_{s}$ projects a $3D$ point in the camera coordinates $\mathbf{X}_{\mathtt{C}} = [X,Y,Z]^T$ into the camera frame pixel $\mathbf{x} = [u_L,v_L,u_R]^T$. 
%
$u_L$ and $v_L$ are respectively the pixel column and row on the left image, and $u_R$ is the pixel column on the right image.

\begin{equation}\label{eqn: stereo_projection}
    \mathbf{x} = \pi_{s}(\mathbf{X}_{\mathtt{C}}) = \begin{bmatrix}
        f_x \frac{X}{Z} + c_x\\
        f_y \frac{Y}{Z} + c_y\\
        f_x \frac{X - b}{Z} + c_x
    \end{bmatrix}
\end{equation}





{\color{red}Revise next part. Use same notation}
We can analyze the computational cost of solving $\mathbf{H}\mathbf{x}=\mathbf{b}$. The Hessian matrix $\mathbf{H}$ can be described as:
\begin{equation}
\mathbf{H} = \left(\begin{array}{cc|cc}
    \mathbf{H}_{C,C} & \mathbf{H}_{C,O} & \mathbf{H}_{C,Op} & \mathbf{H}_{C,Mp} \\
    \mathbf{H}_{O,C} & \mathbf{H}_{O,O} & \mathbf{H}_{O,Op} & \mathbf{H}_{O,Mp} \\
    \hline
    \mathbf{H}_{Op,C} & \mathbf{H}_{Op,O} & \mathbf{H}_{Op,Op} & \mathbf{H}_{Op,Mp} \\
    \mathbf{H}_{Mp,C} & \mathbf{H}_{Mp,O} & \mathbf{H}_{Mp,Op} & \mathbf{H}_{Mp,Mp} \\
\end{array}\right) = \left(\begin{array}{cc}
    \mathbf{H}_{CO,CO} & \mathbf{H}_{CO,P} \\ \mathbf{H}_{P,CO} & \mathbf{H}_{P,P}
\end{array}\right)
\end{equation}
According to figure \ref{fig: hessianBA}, matrix blocks:
\begin{itemize}
    \item $\mathbf{H}_{C,C}$, $\mathbf{H}_{O,O}$, $\mathbf{H}_{Op,Op}$ and $\mathbf{H}_{Mp,Mp}$ have a diagonal structure.
    \item $\mathbf{H}_{C,Op}$, $\mathbf{H}_{C,Mp}$, $\mathbf{H}_{O,Op}$ and their transpose blocks are dense matrices.
    \item $\mathbf{H}_{C,O}$ and its transpose block are sparse matrices.
    \item $\mathbf{H}_{O,Mp}$, $\mathbf{H}_{Op,Mp}$ and their transpose blocks are zero matrices.
\end{itemize}
The gradient vector is:
\begin{equation}
\mathbf{b} = \left(\begin{array}{c}
    \mathbf{b}_{C} \\
    \mathbf{b}_{O} \\ \hline
    \mathbf{b}_{Op} \\
    \mathbf{b}_{Mp}
\end{array}\right) = \left(\begin{array}{c}
    \mathbf{b}_{CO} \\
    \mathbf{b}_{P}
\end{array}\right)
\end{equation}
Being fully dense, where $\mathbf{b}_{C} \in \mathbb{R}^{N_C}$, $\mathbf{b}_{O} \in \mathbb{R}^{N_O}$, $\mathbf{b}_{Mp} \in \mathbb{R}^{N_{Mp}}$ and $\mathbf{b}_{Op} \in \mathbb{R}^{N_{Op}}$. We also define the next terms $N_{CO} = N_C + N_O$ and $N_P = N_{Mp} + N_{Op}$. The variable vector is:
\begin{equation}
\mathbf{x} = \left(\begin{array}{c}
    \mathbf{x}_{C} \\
    \mathbf{x}_{O} \\ \hline
    \mathbf{x}_{Op} \\
    \mathbf{x}_{Mp}
\end{array}\right) = \left(\begin{array}{c}
    \mathbf{x}_{CO} \\
    \mathbf{x}_{P}
\end{array}\right)
\end{equation}
Solving $\mathbf{H}\mathbf{x}=\mathbf{b}$ with Schur complement consists on:
\begin{enumerate}
\item Reduce system: In this case we are going to reduce Object Points (Op) and Map Points (Mp) since they are supposed to be much greater than Camera and Object variables. This step consists on computing:
    \begin{equation}
    \label{eq:reducedH}
        \mathbf{H}' = (\mathbf{H}_{CO,CO}-\mathbf{H}_{CO,P}\mathbf{H}_{P,P}^{-1}\mathbf{H}_{P,CO})
    \end{equation}
    \begin{equation}
    \label{eq:reducedb}
        \mathbf{b}' = (\mathbf{b}_{CO}-\mathbf{H}_{CO,P}\mathbf{H}_{P,P}^{-1}\mathbf{b}_{P})
    \end{equation}
    Taking into account matrix block properties, cost of computing equation \ref{eq:reducedH} are:
    \begin{itemize}
        \item $\mathbf{H}_{P,P}^{-1}$ matrix inversion has cost $\mathcal{O}(N_P)$
        \item $\mathbf{H}_{P,P}^{-1}*\mathbf{H}_{P,CO}$ matrix multiplication has cost $\mathcal{O}(N_{CO}N_P)$
        \item $\mathbf{H}_{CO,P}*(\mathbf{H}_{P,P}^{-1}\mathbf{H}_{P,CO})$ matrix multiplication has cost $\mathcal{O}(N_C^3 + N_C^2 N_{Mp} + N_C N_O N_{Op})$ (TODO check, last term should be $N_C N_O N_{Op} / num_{Obj}$ see block $\mathbf{H}_{O,Op}$)
        \item $(\mathbf{H}_{CO,CO}-\mathbf{H}_{CO,P}\mathbf{H}_{P,P}^{-1}\mathbf{H}_{P,CO})$ matrix sum $\mathcal{O}(N_C^2)$
    \end{itemize}
    
    while equation \ref{eq:reducedb}:
    \begin{itemize}
        \item $\mathbf{H}_{P,P}^{-1}\mathbf{b}_{P}$ is $\mathcal{O}(N_P)$
        \item $\mathbf{H}_{CO,P}\mathbf{H}_{P,P}^{-1}\mathbf{b}_{P}$ is $\mathcal{O}(N_{CO} N_P + N_{O} N_{Op})$ (TODO check, last term should be $N_O N_{Op} / num_{Obj}$ see block $\mathbf{H}_{O,Op}$)
        \item $\mathbf{H}_{CO,P}\mathbf{H}_{P,P}^{-1}\mathbf{b}_{P}$ is $\mathcal{O}(N_P)$
    \end{itemize}
\item Solve reduce system:
    \begin{equation}
        \mathbf{x}_{CO} = (\mathbf{H}')^{-1} \mathbf{b}'
    \end{equation}
    This step has overall cost $\mathcal{O}(N_{CO}^3)$
\item Compute reduced variables:
    \begin{equation}
        \mathbf{x}_{P} = \mathbf{H}_{P,P}^{-1}(\mathbf{b}_{P}-\mathbf{H}_{P,CO} \mathbf{x}_{CO})
    \end{equation}
    TODO write cost
\end{enumerate}
Solving the full system with Schur complement has cost $\mathcal{O}(N_C^3 + N_C^2 N_{Mp} + N_C N_O N_{Op})$. Depending on the number of fixed and dynamic points, the cost will be dominated by $N_C^2 N_{Mp}$ or $N_C N_O N_{Op}$




The derivative of the term $\Delta \mathbf{T}_{\mathtt{O}_k}^{i,i+1}(\mathbf{w}^k_i, \mathbf{v}^k_i)$ with respect to the angular velocity is approximated as follows. 
%
Let us apply an additive perturbation $\delta \mathbf{w}^k_i$ to the object angular velocity (Eqn.~\ref{eqn: delta_w}). 
%
We write only the rotational part of the pose transformation for simplicity.

\begin{equation} \label{eqn: delta_w}
\Delta \mathbf{R}_{\mathtt{O}_k}^{i,i+1} (\mathbf{w}^k_i + \delta \mathbf{w}^k_i) = 
    \text{Exp}((\mathbf{w}^k_i + \delta \mathbf{w}^k_i)\Delta t) 
\end{equation}

We use the first order approximation (Eqn.~\ref{eqn: taylor}), where the term $\mathbf{J}_r$ is the right Jacobian of $\text{SO}(3)$ (\cite{forster2016manifold}) and
relates additive increments in the tangent space to multiplicative
increments applied on the right-hand side

\begin{equation} \label{eqn: taylor}
\Delta \mathbf{R}_{\mathtt{O}_k}^{i,i+1} (\mathbf{w}^k_i + \delta \mathbf{w}^k_i) \approx
    \text{Exp}(\mathbf{w}^k_i \Delta t) \text{Exp}(\mathbf{J}_r(\mathbf{w}^k_i \Delta t)\delta \mathbf{w}^k_i \Delta t) 
\end{equation}

Assuming that the term $\mathbf{J}_r(\mathbf{w}^k_i \Delta t) \delta \mathbf{w}^k_i \Delta t$ is small, we can rewrite the equation as:

\begin{equation} \label{eqn: Jr_small}
\Delta \mathbf{R}_{\mathtt{O}_k}^{i,i+1} (\mathbf{w}^k_i + \delta \mathbf{w}^k_i) \approx
    \text{Exp}(\mathbf{w}^k_i \Delta t) (\mathbf{I} + [\mathbf{J}_r(\mathbf{w}^k_i \Delta t)\delta \mathbf{w}^k_i \Delta t]_\times),
\end{equation}

where $[\cdot]_\times$ is the skew operator that transforms a vector in $\mathbb{R}^3$ into a skew symmetric matrix. 
%
Therefore, the partial derivative of $\Delta \mathbf{R}_{\mathtt{O}_k}^{i,i+1}$ with respect to the angular velocity can be written as follows:

\begin{equation} \label{eqn: partial}
\frac{\partial \Delta \mathbf{R}_{\mathtt{O}_k}^{i,i+1}}{\partial \delta \mathbf{w}^k_i} = \text{Exp}(\mathbf{w}^k_i \Delta t) [\mathbf{J}_r(\mathbf{w}^k_i \Delta t) \Delta t]_\times
\end{equation}

\begin{table} [t]
\footnotesize
\begin{tabularx}{\linewidth}{@{}l*{10}{C}}
\toprule
\multicolumn{1}{c|}{seq} & \multicolumn{3}{c|}{ORB-SLAM~\cite{mur2015orb}} & \multicolumn{3}{c|}{DynaSLAM~\cite{bescos2018dynaslam}} & \multicolumn{3}{c}{Ours}
\\
\multicolumn{1}{c|}{} & ATE & RPE\textsubscript{t} & \multicolumn{1}{c|}{RPE\textsubscript{R}} & ATE & RPE\textsubscript{t} & \multicolumn{1}{c|}{RPE\textsubscript{R}} & ATE & RPE\textsubscript{t} & \multicolumn{1}{c}{RPE\textsubscript{R}}
\\
\midrule
\multicolumn{1}{c|}{00} & \textbf{1.38} & \textbf{1.30} & \multicolumn{1}{c|}{\textbf{0.90}} & 1.43 & 1.32 & \multicolumn{1}{c|}{0.92} & 1.55 & 1.45 & \multicolumn{1}{c}{0.99} 
\\
\multicolumn{1}{c|}{01} & 10.79 & 1.89 & \multicolumn{1}{c|}{\textbf{0.40}} & \textbf{9.74} & \textbf{1.87} & \multicolumn{1}{c|}{\textbf{0.40}} & 10.16 & 1.90 & \multicolumn{1}{c}{0.48} 
\\
\multicolumn{1}{c|}{02} & \textbf{5.59} & \textbf{1.15} & \multicolumn{1}{c|}{\textbf{0.51}} & 6.75 & 1.28 & \multicolumn{1}{c|}{0.74} & 7.85 & 1.36 & \multicolumn{1}{c}{0.91} 
\\
\multicolumn{1}{c|}{03} & \textbf{0.64} & \textbf{0.77} & \multicolumn{1}{c|}{0.38} & 0.65 & 0.78 & \multicolumn{1}{c|}{0.36} & 0.88 & 1.00 & \multicolumn{1}{c}{\textbf{0.31}}
\\
\multicolumn{1}{c|}{04} & 0.85 & 1.22 & \multicolumn{1}{c|}{0.60} & 0.78 & 1.10 & \multicolumn{1}{c|}{0.52} & \textbf{0.32} & \textbf{0.72} & \multicolumn{1}{c}{\textbf{0.23}} 
\\
\multicolumn{1}{c|}{05} & 0.72 & \textbf{0.74} & \multicolumn{1}{c|}{\textbf{0.42}} & \textbf{0.71} & 0.75 & \multicolumn{1}{c|}{0.43} & 0.89 & 0.80 & \multicolumn{1}{c}{0.46} 
\\
\multicolumn{1}{c|}{06} & 0.57 & 0.73 & \multicolumn{1}{c|}{\textbf{0.37}} & \textbf{0.56} & 0.69 & \multicolumn{1}{c|}{0.41} & 0.72 & \textbf{0.63} & \multicolumn{1}{c}{0.65} 
\\
\multicolumn{1}{c|}{07} & 0.56 & \textbf{0.76} & \multicolumn{1}{c|}{0.60} & 0.56 & 0.77 & \multicolumn{1}{c|}{\textbf{0.58}} & \textbf{0.47} & 0.93 & \multicolumn{1}{c}{0.76} 
\\
\multicolumn{1}{c|}{08} & \textbf{3.58} & \textbf{1.79} & \multicolumn{1}{c|}{\textbf{0.69}} & 4.21 & 1.80 & \multicolumn{1}{c|}{0.71} & \textbf{3.58} & 1.87 & \multicolumn{1}{c}{0.71} 
\\
\multicolumn{1}{c|}{09} & 2.90 & \textbf{1.01} & \multicolumn{1}{c|}{\textbf{0.41}} & 3.33 & 1.02 & \multicolumn{1}{c|}{0.50} & \textbf{2.12} & 1.12 & \multicolumn{1}{c}{0.64} 
\\
\multicolumn{1}{c|}{10} & \textbf{1.27} & 0.99 & \multicolumn{1}{c|}{\textbf{0.58}} & \textbf{1.27} & \textbf{0.97} & \multicolumn{1}{c|}{\textbf{0.58}} & 1.58 & 0.99 & \multicolumn{1}{c}{0.60} 
\\
\bottomrule
\end{tabularx}
\caption{\label{tab: egomotion_KITTI_odometry} Results on the KITTI \underline{odometry} dataset. 
%
The ATE, RPE\textsubscript{t} and RPE\textsubscript{R} are given in m, m/100m and \degree/100m.}
\end{table}

\begin{table*}[t]
\scriptsize
\begin{tabularx}{\linewidth}{@{}l*{13}{C}}
\toprule
\multicolumn{2}{c|}{sequence} & \multicolumn{2}{c|}{$0003$} & \multicolumn{1}{c|}{$0006$} & \multicolumn{1}{c|}{$0010$} & \multicolumn{1}{1|}{$0017$} & \multicolumn{3}{c|}{$0018$} & \multicolumn{4}{c}{$0020$}
\\
\multicolumn{2}{c|}{object id (class)} & $0$ (car) & \multicolumn{1}{c|}{$1$ (car)} & \multicolumn{1}{c|}{$4$ (car)} & \multicolumn{1}{c|}{$0$ (car)} & \multicolumn{1}{c|}{$6$ (person)} & $1$ (car) & $2$ (car) & \multicolumn{1}{c|}{$3$ (car)} & $0$ (car) & $2$ (car) & $3$ (car) & $9$ (car)
\\
\midrule
\multicolumn{2}{c|}{ATE~[$m$]} & 0.95 & \multicolumn{1}{c|}{0.69} & \multicolumn{1}{c|}{2.42} & \multicolumn{1}{c|}{0.95} & \multicolumn{1}{c|}{0.57} & 0.70 & 1.10 & \multicolumn{1}{c|}{1.13} & 0.56 & 0.77 & 0.23 & 0.58
\\
\multicolumn{2}{c|}{RPE_t~[$m/m$]} & 0.28 & \multicolumn{1}{c|}{0.34} & \multicolumn{1}{c|}{0.90} & \multicolumn{1}{c|}{0.40} & \multicolumn{1}{c|}{1.25} & 0.45 & 0.30 & \multicolumn{1}{c|}{0.55} & 0.45 & 0.69 & 0.23 & 0.36
\\
\multicolumn{2}{c|}{RPE_R~[$\degree/m$]} & 3.07 & \multicolumn{1}{c|}{1.84} & \multicolumn{1}{c|}{2.46} & \multicolumn{1}{c|}{2.84} & \multicolumn{1}{c|}{37.47} & 11.72 & 9.27 & \multicolumn{1}{c|}{20.05} & 1.30 & 10.18 & 0.93 & 1.62
\\
\midrule
\midrule
% \multirow{3}{*}{2D} & \multicolumn{1}{c|}{\# TP} & 48 & \multicolumn{1}{c|}{50} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c|}{163} & \multicolumn{1}{c|}{65} & 100 & 189 & \multicolumn{1}{c|}{160} & 122 & 36 & 61 & 88
% \\
\multirow{2}{*}{2D} & \multicolumn{1}{c|}{TP (\%)} & 77.63 & \multicolumn{1}{c|}{52.46} & \multicolumn{1}{c|}{91.49} & \multicolumn{1}{c|}{81.63} & \multicolumn{1}{c|}{74.48} & 75.79 & 86.74 & \multicolumn{1}{c|}{53.33} & 64.68 & 100.00 & 100.0 & 92.55
\\
& \multicolumn{1}{c|}{MOTP~[$\%$]} & 86.99 & \multicolumn{1}{c|}{77.55} & \multicolumn{1}{c|}{78.08} & \multicolumn{1}{c|}{73.51} & \multicolumn{1}{c|}{64.33} & 93.43 & 80.42 & \multicolumn{1}{c|}{76.60} & 78.54 & 70.19 & 84.33 & 75.87
\\
\midrule
% \multirow{3}{*}{BV} & \multicolumn{1}{c|}{\# TP} & 48 & \multicolumn{1}{c|}{48} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c|}{135} & \multicolumn{1}{c|}{24} & 75 & 150 & \multicolumn{1}{c|}{92} & 120 & 36 & 67 & 88
% \\
\multirow{2}{*}{BV} & \multicolumn{1}{c|}{TP (\%)} & 75.00 & \multicolumn{1}{c|}{43.11} & \multicolumn{1}{c|}{92.5} & \multicolumn{1}{c|}{52.38} & \multicolumn{1}{c|}{17.93} & 62.24 & 67.05 & \multicolumn{1}{c|}{37.89} & 43.78 & 60.00 & 100.0 & 92.05
\\
& \multicolumn{1}{c|}{MOTP~[$\%$]} & 73.88 & \multicolumn{1}{c|}{74.00} & \multicolumn{1}{c|}{62.29} & \multicolumn{1}{c|}{53.01} & \multicolumn{1}{c|}{31.61} & 69.77 & 45.47 & \multicolumn{1}{c|}{41.45} & 44.99 & 48.08 & 84.70 & 57.80
\\
\midrule
% \multirow{3}{*}{3D} & \multicolumn{1}{c|}{\# TP} & 48 & \multicolumn{1}{c|}{48} & \multicolumn{1}{c|}{25} & \multicolumn{1}{c|}{124} & \multicolumn{1}{c|}{0} & 57 & 125 & \multicolumn{1}{c|}{63} & 110 & 30 & 67 & 83
% \\
\multirow{2}{*}{3D} & \multicolumn{1}{c|}{TP (\%)} & 75.00 & \multicolumn{1}{c|}{42.20} & \multicolumn{1}{c|}{90.00} & \multicolumn{1}{c|}{50.00} & \multicolumn{1}{c|}{0.00} & 62.24 & 61.36 & \multicolumn{1}{c|}{35.08} & 31.84 & 55.55 & 100.00 & 79.55
\\
& \multicolumn{1}{c|}{MOTP~[$\%$]} & 60.13 & \multicolumn{1}{c|}{61.49} & \multicolumn{1}{c|}{46.45} & \multicolumn{1}{c|}{44.97} & \multicolumn{1}{c|}{0.00} & 48.13 & 41.84 & \multicolumn{1}{c|}{43.85} & 46.15 & 39.29 & 69.64 & 52.53
\\
\bottomrule
\end{tabularx}
\caption[Objects motion evaluation on the KITTI tracking dataset]{\label{tab: object_tracking_trajectories} Objects motion comparison on the KITTI \underline{tracking} dataset.}
\end{table*}

==> graphs/num_parameters_nc.tex <==
\begin{tikzpicture}

\begin{axis}[%
width=2.2in,
height=1.5in,
scale only axis,
xmin=0,
xmax=50,
xlabel style={font=\footnotesize},
xlabel={Points per object},
ymin=0,
ymax=2.25,
ylabel style={font=\footnotesize},
ylabel={Compression ratio},
axis background/.style={fill=white},
tick label style={font=\footnotesize},
legend style={legend pos=north east, font=\footnotesize}
]
\addplot [color=cyan, line width=1.5pt]
  table[row sep=crcr]{%
    1.00 1.00 \\ 
     2.00 1.00 \\ 
     3.00 1.00 \\ 
     4.00 1.00 \\ 
     5.00 1.00 \\ 
     6.00 1.00 \\ 
     7.00 1.00 \\ 
     8.00 1.00 \\ 
     9.00 1.00 \\ 
     10.00 1.00 \\ 
     11.00 1.00 \\ 
     12.00 1.00 \\ 
     13.00 1.00 \\ 
     14.00 1.00 \\ 
     15.00 1.00 \\ 
     16.00 1.00 \\ 
     17.00 1.00 \\ 
     18.00 1.00 \\ 
     19.00 1.00 \\ 
     20.00 1.00 \\ 
     21.00 1.00 \\ 
     22.00 1.00 \\ 
     23.00 1.00 \\ 
     24.00 1.00 \\ 
     25.00 1.00 \\ 
     26.00 1.00 \\ 
     27.00 1.00 \\ 
     28.00 1.00 \\ 
     29.00 1.00 \\ 
     30.00 1.00 \\ 
     31.00 1.00 \\ 
     32.00 1.00 \\ 
     33.00 1.00 \\ 
     34.00 1.00 \\ 
     35.00 1.00 \\ 
     36.00 1.00 \\ 
     37.00 1.00 \\ 
     38.00 1.00 \\ 
     39.00 1.00 \\ 
     40.00 1.00 \\ 
     41.00 1.00 \\ 
     42.00 1.00 \\ 
     43.00 1.00 \\ 
     44.00 1.00 \\ 
     45.00 1.00 \\ 
     46.00 1.00 \\ 
     47.00 1.00 \\ 
     48.00 1.00 \\ 
     49.00 1.00 \\ 
     50.00 1.00 \\ 
     51.00 1.00 \\ 
     52.00 1.00 \\ 
     53.00 1.00 \\ 
     54.00 1.00 \\ 
     55.00 1.00 \\ 
     56.00 1.00 \\ 
     57.00 1.00 \\ 
     58.00 1.00 \\ 
     59.00 1.00 \\ 
     60.00 1.00 \\ 
     61.00 1.00 \\ 
     62.00 1.00 \\ 
     63.00 1.00 \\ 
     64.00 1.00 \\ 
     65.00 1.00 \\ 
     66.00 1.00 \\ 
     67.00 1.00 \\ 
     68.00 1.00 \\ 
     69.00 1.00 \\ 
     70.00 1.00 \\ 
     71.00 1.00 \\ 
     72.00 1.00 \\ 
     73.00 1.00 \\ 
     74.00 1.00 \\ 
     75.00 1.00 \\ 
     76.00 1.00 \\ 
     77.00 1.00 \\ 
     78.00 1.00 \\ 
     79.00 1.00 \\ 
     80.00 1.00 \\ 
     81.00 1.00 \\ 
     82.00 1.00 \\ 
     83.00 1.00 \\ 
     84.00 1.00 \\ 
     85.00 1.00 \\ 
     86.00 1.00 \\ 
     87.00 1.00 \\ 
     88.00 1.00 \\ 
     89.00 1.00 \\ 
     90.00 1.00 \\ 
     91.00 1.00 \\ 
     92.00 1.00 \\ 
     93.00 1.00 \\ 
     94.00 1.00 \\ 
     95.00 1.00 \\ 
     96.00 1.00 \\ 
     97.00 1.00 \\ 
     98.00 1.00 \\ 
     99.00 1.00 \\ 
     100.00 1.00 \\ 
};

\addlegendentry{No objects}

\addplot [color=red, dotted, line width=1.5pt]
  table[row sep=crcr]{%
    1.00 2.05 \\
     2.00 1.05 \\
     3.00 0.72 \\
     4.00 0.55 \\
     5.00 0.45 \\
     6.00 0.38 \\
     7.00 0.34 \\
     8.00 0.30 \\
     9.00 0.27 \\
     10.00 0.25 \\
     11.00 0.23 \\
     12.00 0.22 \\
     13.00 0.20 \\
     14.00 0.19 \\
     15.00 0.18 \\
     16.00 0.17 \\
     17.00 0.17 \\
     18.00 0.16 \\
     19.00 0.16 \\
     20.00 0.15 \\
     21.00 0.15 \\
     22.00 0.14 \\
     23.00 0.14 \\
     24.00 0.13 \\
     25.00 0.13 \\
     26.00 0.13 \\
     27.00 0.12 \\
     28.00 0.12 \\
     29.00 0.12 \\
     30.00 0.12 \\
     31.00 0.11 \\
     32.00 0.11 \\
     33.00 0.11 \\
     34.00 0.11 \\
     35.00 0.11 \\
     36.00 0.11 \\
     37.00 0.10 \\
     38.00 0.10 \\
     39.00 0.10 \\
     40.00 0.10 \\
     41.00 0.10 \\
     42.00 0.10 \\
     43.00 0.10 \\
     44.00 0.10 \\
     45.00 0.09 \\
     46.00 0.09 \\
     47.00 0.09 \\
     48.00 0.09 \\
     49.00 0.09 \\
     50.00 0.09 \\
     51.00 0.09 \\
     52.00 0.09 \\
     53.00 0.09 \\
     54.00 0.09 \\
     55.00 0.09 \\
     56.00 0.09 \\
     57.00 0.09 \\
     58.00 0.08 \\
     59.00 0.08 \\
     60.00 0.08 \\
     61.00 0.08 \\
     62.00 0.08 \\
     63.00 0.08 \\
     64.00 0.08 \\
     65.00 0.08 \\
     66.00 0.08 \\
     67.00 0.08 \\
     68.00 0.08 \\
     69.00 0.08 \\
     70.00 0.08 \\
     71.00 0.08 \\
     72.00 0.08 \\
     73.00 0.08 \\
     74.00 0.08 \\
     75.00 0.08 \\
     76.00 0.08 \\
     77.00 0.08 \\
     78.00 0.08 \\
     79.00 0.08 \\
     80.00 0.07 \\
     81.00 0.07 \\
     82.00 0.07 \\
     83.00 0.07 \\
     84.00 0.07 \\
     85.00 0.07 \\
     86.00 0.07 \\
     87.00 0.07 \\
     88.00 0.07 \\
     89.00 0.07 \\
     90.00 0.07 \\
     91.00 0.07 \\
     92.00 0.07 \\
     93.00 0.07 \\
     94.00 0.07 \\
     95.00 0.07 \\
     96.00 0.07 \\
     97.00 0.07 \\
     98.00 0.07 \\
     99.00 0.07 \\
     100.00 0.07 \\
};

\addlegendentry{$N_o = 1$}
    
\addplot [color=green, dash dot, line width=1.5pt]
  table[row sep=crcr]{% 
    1.00 1.25 \\
     2.00 0.65 \\
     3.00 0.45 \\
     4.00 0.35 \\
     5.00 0.29 \\
     6.00 0.25 \\
     7.00 0.22 \\
     8.00 0.20 \\
     9.00 0.18 \\
     10.00 0.17 \\
     11.00 0.16 \\
     12.00 0.15 \\
     13.00 0.14 \\
     14.00 0.14 \\
     15.00 0.13 \\
     16.00 0.13 \\
     17.00 0.12 \\
     18.00 0.12 \\
     19.00 0.11 \\
     20.00 0.11 \\
     21.00 0.11 \\
     22.00 0.10 \\
     23.00 0.10 \\
     24.00 0.10 \\
     25.00 0.10 \\
     26.00 0.10 \\
     27.00 0.09 \\
     28.00 0.09 \\
     29.00 0.09 \\
     30.00 0.09 \\
     31.00 0.09 \\
     32.00 0.09 \\
     33.00 0.09 \\
     34.00 0.09 \\
     35.00 0.08 \\
     36.00 0.08 \\
     37.00 0.08 \\
     38.00 0.08 \\
     39.00 0.08 \\
     40.00 0.08 \\
     41.00 0.08 \\
     42.00 0.08 \\
     43.00 0.08 \\
     44.00 0.08 \\
     45.00 0.08 \\
     46.00 0.08 \\
     47.00 0.08 \\
     48.00 0.07 \\
     49.00 0.07 \\
     50.00 0.07 \\
     51.00 0.07 \\
     52.00 0.07 \\
     53.00 0.07 \\
     54.00 0.07 \\
     55.00 0.07 \\
     56.00 0.07 \\
     57.00 0.07 \\
     58.00 0.07 \\
     59.00 0.07 \\
     60.00 0.07 \\
     61.00 0.07 \\
     62.00 0.07 \\
     63.00 0.07 \\
     64.00 0.07 \\
     65.00 0.07 \\
     66.00 0.07 \\
     67.00 0.07 \\
     68.00 0.07 \\
     69.00 0.07 \\
     70.00 0.07 \\
     71.00 0.07 \\
     72.00 0.07 \\
     73.00 0.07 \\
     74.00 0.07 \\
     75.00 0.07 \\
     76.00 0.07 \\
     77.00 0.07 \\
     78.00 0.07 \\
     79.00 0.07 \\
     80.00 0.07 \\
     81.00 0.06 \\
     82.00 0.06 \\
     83.00 0.06 \\
     84.00 0.06 \\
     85.00 0.06 \\
     86.00 0.06 \\
     87.00 0.06 \\
     88.00 0.06 \\
     89.00 0.06 \\
     90.00 0.06 \\
     91.00 0.06 \\
     92.00 0.06 \\
     93.00 0.06 \\
     94.00 0.06 \\
     95.00 0.06 \\
     96.00 0.06 \\
     97.00 0.06 \\
     98.00 0.06 \\
     99.00 0.06 \\
     100.00 0.06 \\ 
};

\addlegendentry{$N_o = 5$}
     
    
\addplot [color=magenta, dashed, line width=1.5pt]
  table[row sep=crcr]{% 
    1.00 1.15 \\
     2.00 0.60 \\
     3.00 0.42 \\
     4.00 0.33 \\
     5.00 0.27 \\
     6.00 0.23 \\
     7.00 0.21 \\
     8.00 0.19 \\
     9.00 0.17 \\
     10.00 0.16 \\
     11.00 0.15 \\
     12.00 0.14 \\
     13.00 0.13 \\
     14.00 0.13 \\
     15.00 0.12 \\
     16.00 0.12 \\
     17.00 0.11 \\
     18.00 0.11 \\
     19.00 0.11 \\
     20.00 0.10 \\
     21.00 0.10 \\
     22.00 0.10 \\
     23.00 0.10 \\
     24.00 0.10 \\
     25.00 0.09 \\
     26.00 0.09 \\
     27.00 0.09 \\
     28.00 0.09 \\
     29.00 0.09 \\
     30.00 0.09 \\
     31.00 0.09 \\
     32.00 0.08 \\
     33.00 0.08 \\
     34.00 0.08 \\
     35.00 0.08 \\
     36.00 0.08 \\
     37.00 0.08 \\
     38.00 0.08 \\
     39.00 0.08 \\
     40.00 0.08 \\
     41.00 0.08 \\
     42.00 0.08 \\
     43.00 0.08 \\
     44.00 0.07 \\
     45.00 0.07 \\
     46.00 0.07 \\
     47.00 0.07 \\
     48.00 0.07 \\
     49.00 0.07 \\
     50.00 0.07 \\
     51.00 0.07 \\
     52.00 0.07 \\
     53.00 0.07 \\
     54.00 0.07 \\
     55.00 0.07 \\
     56.00 0.07 \\
     57.00 0.07 \\
     58.00 0.07 \\
     59.00 0.07 \\
     60.00 0.07 \\
     61.00 0.07 \\
     62.00 0.07 \\
     63.00 0.07 \\
     64.00 0.07 \\
     65.00 0.07 \\
     66.00 0.07 \\
     67.00 0.07 \\
     68.00 0.07 \\
     69.00 0.07 \\
     70.00 0.07 \\
     71.00 0.07 \\
     72.00 0.07 \\
     73.00 0.07 \\
     74.00 0.06 \\
     75.00 0.06 \\
     76.00 0.06 \\
     77.00 0.06 \\
     78.00 0.06 \\
     79.00 0.06 \\
     80.00 0.06 \\
     81.00 0.06 \\
     82.00 0.06 \\
     83.00 0.06 \\
     84.00 0.06 \\
     85.00 0.06 \\
     86.00 0.06 \\
     87.00 0.06 \\
     88.00 0.06 \\
     89.00 0.06 \\
     90.00 0.06 \\
     91.00 0.06 \\
     92.00 0.06 \\
     93.00 0.06 \\
     94.00 0.06 \\
     95.00 0.06 \\
     96.00 0.06 \\
     97.00 0.06 \\
     98.00 0.06 \\
     99.00 0.06 \\
     100.00 0.06 \\
};
     
\addlegendentry{$N_o = 10$}
     
     
\end{axis}
\end{tikzpicture}%
